HarDNN: Feature Map Vulnerability Evaluation in CNNs

As Convolutional Neural Networks (CNNs) are increasingly being employed in safety-critical applications, it is important that they behave reliably in the face of hardware errors. Transient hardware errors may percolate undesirable state during execution, resulting in software-manifested errors which can adversely affect high-level decision making. This paper presents HarDNN, a software-directed approach to identify vulnerable computations during a CNN inference and selectively protect them based on their propensity towards corrupting the inference output in the presence of a hardware error. We show that HarDNN can accurately estimate relative vulnerability of a feature map (fmap) in CNNs using a statistical error injection campaign, and explore heuristics for fast vulnerability assessment. Based on these results, we analyze the tradeoff between error coverage and computational overhead that the system designers can use to employ selective protection. Results show that the improvement in resilience for the added computation is superlinear with HarDNN. For example, HarDNN improves SqueezeNet's resilience by 10x with just 30% additional computations.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\input{./figures/layer_fig.tex}

This section provides insights on higher level aspects of CNN vulnerability, guided by HarDNN's techniques. Intro... sentences

Although HarDNN focuses on feature map vulnerability analysis for multiple reasons (section X), one benefit of Fmap analysis
is that it is composable to study layer-level vulnerability.

Figure~\ref{fig:layer_analysis} plots percentage of errors (mismatches) observed for each conv layer in the network. We can
gather various insights from this figure:

0) Better trained networks show lower error rates (resnet, vgg, mobilenet) vs others

1) Overall error percentage in networks is low (look at the Y-axis). 

2) On average, earlier layers are more vulnerable than later layers. This also is in agreement with prior work (SC '17). Except mobileNet..

3) Jagged lines: num of feature maps (note mobilenet has a sudden surge in filters/feature map by design in the later layers)
(if we can validate it) CONV-->CONV-->RELU vs CONV-->RELU. In general, RELU is good because it masks errors (whether or not we do this in our experiments...)

Although, better trained networks have observe fewer errors, it is not clear that networks with the same training accuracy 
necessarily have the same overall vulnerability. We observe this in figure 8, since we see that GoogleNet on average has
lower per-layer error rates than shufflenet, although both observe similar accuracy (Table 1).

To quantify this, we compute the average vulnerability of the network, but finding the weighted product of 
the layer and mismatch rate. (in other words, combining points 1 and 3 above). Table XX shows the results...

This will be computed as: 
totalNetworkVulnerability = 0
for Layer in Network:
    LayerVulnerability = totalFmaps[Layer]*errorProbability[Layer]
    totalNetworkVulnerability += LayerVulnerability  % sum

(should we do sum or average for the table?)


Thus: similar accuracy, but different vulnerability




% A) 
% Accuracy of the network --> lower error rate

% Takeaway: better trained networks produce fewer errors

% \Comment{Siva: (A.1) Confidence of the classification -> SDC probability.}

% B) 
% Early vs. Late Layers: 

% \Comment{Siva: Graph showing the vulnerability of different layers. Plot vulnerability on y-axis and layer count on x-axis. One graph for all the networks we studied.}


% C)
% Layer type: skip connections immune? BN: smaller dynamic range (and improve accuracy)?


% \Comment{Siva: I think this section will add a lot of value to the paper.}

==> tables/error_models_table.tex <==
\begin{table}[t]
    \caption{Error Models}
	%\fontsize{8}{10}\selectfont
	\scriptsize
     	\centering
        \renewcommand{\arraystretch}{1.0}
            \begin{tabular}{|c|c|c|c|}
                    \hline
                      \textbf{Name} & \textbf{Format} & \textbf{Quantized?} & \textbf{Description} \\
                    \hline\hline
                    FP-Rand & Floating-point & No & Random value  \\
                    & & & from [-max, max] \\
                    \hline
                    FxP-Rand & Fixed-point & Yes & Random quantized \\
                    & & & value from [-max, max] \\
                    \hline
                    FxP-Flip & Fixed-point & Yes & Random bit flip \\
                    % & Point & & \\
                    \hline
        \end{tabular}

\label{table:error_models}
\end{table}
%\vspace{-.2in}
